Feature Partitioning for Robust Tree Ensembles and their Certification in Adversarial Scenarios

Machine learning algorithms, however effective, are known to be vulnerable in adversarial scenarios where a malicious user may inject manipulated instances. In this work we focus on evasion attacks, where a model is trained in a safe environment and exposed to attacks at test time. The attacker aims at finding a minimal perturbation of a test instance that changes the model outcome. We propose a model-agnostic strategy that builds a robust ensemble by training its basic models on feature-based partitions of the given dataset. Our algorithm guarantees that the majority of the models in the ensemble cannot be affected by the attacker. We experimented the proposed strategy on decision tree ensembles, and we also propose an approximate certification method for tree ensembles that efficiently assess the minimal accuracy of a forest on a given dataset avoiding the costly computation of evasion attacks. Experimental evaluation on publicly available datasets shows that proposed strategy outperforms state-of-the-art adversarial learning algorithms against evasion attacks.

==> 04-exp.tex <==
%!TEX root=./paper.tex

\section{Experiments}
\label{sec:exp}

\todocla{Robusteness of a robust forest on varying number of trees}

\todocla{Accuracy of heuristic evaluation}

\todocla{Accuracy of proposed algorithm}


\todocla{Analisys with lower bounds}


\begin{table}[t]
\caption{Datasets description.}
\label{dataset-table}
\scriptsize
\vskip 0.15in
\begin{center}
\begin{sc}
\begin{tabular}{ccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{dataset}} & 
\multicolumn{1}{c}{\multirow{2}{*}{\#feat}} & 
\multicolumn{1}{c}{\multirow{2}{*}{\#imp}} & 
\multicolumn{1}{c}{\multirow{2}{*}{\%clss}} & 
\multicolumn{3}{c}{\#instances} \\
& & & & \#total & \#train & \#test \\
\midrule
Breast & 30 & 15 & 62.7\% & 569 & 375 & 194 \\
Wine 0/12 & 13 & 9 & 66.9 & 178\% & 117 & 61 \\
\bottomrule
\end{tabular}
\end{sc}
\end{center}
\vskip -0.1in
\end{table}



\begin{table*}[t]
\caption{Breast cancer robust accuracy.}
\label{table:breast_cancer_robust}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ccrrlllllll}
\toprule
\multicolumn{4}{c}{Forest parameters} 
& \multicolumn{3}{c}{Attacked features} 
& \multicolumn{2}{c}{Acc lb1} 
& \multicolumn{2}{c}{Acc lb2}\\
mln & B & Rounds & \#tree & 0 & 1 & 2 & 1 & 2 & 1 & 2 \\
\midrule
	\multirow{12}{*}{Inf} & \multirow{3}{*}{1} & 1 & 3 & .969 & .861 & 0 & .861 & 0 & .861 & 0 \\
			     &			     & 10 & 30 & .974 & .907 & .557 & .861 & 0 & .861 & 0 \\
			     &			     & 100 & 300 & .974 & .902 & .701 & .871 & 0 & .866 & 0 \\
			     & \multirow{3}{*}{2} & 1 & 5 & .964 & .918 & .778 & .918 & .778 & .918 & .778 \\
			     &			     & 10 & 50 & .964 & .928 & .851 & .902 & .778 & .902 & .778 \\
			     &			     & 100 & 500 & .964 & .938 & .866 & .923 & .825 & .907 & .773 \\
			     & \multirow{2}{*}{3} & 1 & 7 & .959 & .933 & .851 & .933 & .851 & .933 & .851 \\
			     &			     & 10 & 70 & .964 & .933 & .897 & .928 & .871 & .928 & .861 \\
			     & \multirow{2}{*}{4}& 1 & 9 & .954 & .912 & .866 & .912 & .866 & .912 & .866 \\
			     &			     & 10 & 90 & .948 & .933 & .902 & .928 & .881 & .923 & .871 \\
			     & \multirow{2}{*}{5}& 1 & 11 & .933 & .912 & .871 & .912 & .871 & .912 & .871 \\
			     &			     & 10 & 110 & .954 & .928 & .902 & .923 & .892 & .923 & .881 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


\begin{table*}[t]
\caption{Wine 0/12 robust accuracy.}
\label{table:wine_0_12_robust}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ccrrlllllll}
\toprule
\multicolumn{4}{c}{Forest parameters} 
& \multicolumn{3}{c}{Attacked features} 
& \multicolumn{2}{c}{Acc lb1} 
& \multicolumn{2}{c}{Acc lb2}\\
mln & B & Rounds & \#tree & 0 & 1 & 2 & 1 & 2 & 1 & 2 \\
\midrule
	\multirow{15}{*}{4} & \multirow{3}{*}{1} & 1 & 3 & .984 & .869 & .41 & .869 & 0 & .869 & 0 \\
			     &			     & 10 & 30 & 1 & .869 & .557 & .836 & 0 & .836 & 0 \\
			     &			     & 100 & 300 & .984 & .902 & .525 & .836 & 0 & .836 & 0 \\
			     & \multirow{3}{*}{2} & 1 & 5 & .967 & .885 & .574 & .885 & .492 & .885 & .492 \\
			     &			     & 10 & 50 & .967 & .918 & .754 & .902 & .557 & .902 & .541 \\
			     &			     & 100 & 500 & .984 & .902 & .803 & .885 & .738 & .869 & .623 \\
			     & \multirow{3}{*}{3} & 1 & 7 & .934 & .885 & .721 & .885 & .721 & .885 & .721 \\
			     &			     & 10 & 70 & .951 & .885 & .77 & .852 & .77 & .852 & .77 \\
			     &			     & 100 & 700 & .967 & .885 & .754 & .869 & .738 & .869 & .738 \\
			     & \multirow{3}{*}{4} & 1 & 9 & .934 & .836 & .738 & .836 & .738 & .836 & .738 \\
			     &			     & 10 & 90 & .951 & .869 & .738 & .869 & .721 & .869 & .721 \\
			     &			     & 100 & 900 & .951 & .852 & .754 & .82 & .754 & .82 & .738 \\
			     & \multirow{3}{*}{5} & 1 & 11 & .885 & .836 & .738 & .836 & .738 & .836 & .738 \\
			     &			     & 10 & 110 & .902 & .82 & .738 & .82 & .738 & .82 & .738 \\
			     &			     & 100 & 1100 & .902 & .836 & .721 & .836 & .721 & .836 & .721 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


The table \ref{table:breast_cancer_robust} shows the results obtained by the RobustSplit model on the Breast dataset. The first column, \texttt{MNL}, identifies the maximum number of leaves of each tree in the forest. Field \texttt{B} indicates how many features the model has been trained to be robust. The \texttt{Rounds} field identifies how many rounds have been executed in the training algorithm \ref{alg:robust_split}. \texttt{\#Tree} is the number of final trees in the forest. \texttt{Attacked Features} identify the accuracy of the model with respect to an attack performed on a number of features ranging from  0 to 2 (0 identifies a safe input). \texttt{Acc LB1} and \texttt{Acc LB2} are the accuracy values returned by the two different search algorithms of the lower bound.

\begin{table}[t]
\caption{Breast cancer random forest accuracy.}
\label{table:breast_cancer_random_forest}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{crlll}
\toprule
\multicolumn{2}{c}{Forest parameters} 
& \multicolumn{3}{c}{Attacked features} \\
\multicolumn{2}{c}{\#tree} & 0 & 1 & 2 \\
\midrule
\multirow{6}{*}{set}	 & 3 & .927 & .366 & 0 \\
                    	 & 5 & .976 & .512 & 0 \\
                    	 & 30 & .976 & .707 & .049 \\
                    	 & 50 & 1 & .659 & .049 \\
                    	 & 300 & 1 & .756 & .171 \\
                     	 & 500 & 1 & .78 & .171 \\
\multirow{3}{*}{best cv} & 6 & .951 & .537 & .268 \\
              		 	 & 33 & .976 & .683 & .049 \\
                    	 & 104 & 1 & .756 & .146 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[t]
\caption{Wine 0/12 random forest accuracy.}
\label{table:wine_0_12_forest}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{crllll}
\toprule
\multicolumn{3}{c}{Forest parameters} 
& \multicolumn{3}{c}{Attacked features} \\
mln & \multicolumn{2}{c}{\#tree} & 0 & 1 & 2 \\
\midrule
\multirow{18}{*}{inf} & \multirow{3}{*}{best cv}  &  4 & .967 & .541 & .23 \\
											      &  & 25 & .967 & .803 & .361 \\
                    	                          &  & 100 & .984 & .82 & .361 \\
					  & \multirow{30}{*}{best cv} & 3 & .918 & .525 & 0 \\
					  &                           & 5 & .967 & .689 & 0 \\
					  &                           & 7 & .984 & .705 & .246 \\
					  &                           & 9 & .967 & .689 & .279 \\
					  &                           & 11 & .967 & .754 & .344 \\
					  &                           & 30 & .967 & .803 & .459 \\
					  &                           & 50 & .967 & .77 & .475 \\
					  &                           & 70 & .967 & .836 & .525 \\
					  &                           & 90 & .967 & .852 & .525 \\
					  &                           & 110 & .967 & .836 & .525 \\
					  &                           & 300 & .984 & .82 & .459 \\
					  &                           & 500 & .984 & .787 & .492 \\
					  &                           & 700 & .984 & .738 & .508 \\
					  &                           & 900 & .984 & .721 & .525 \\
					  &                           & 1100 & .984 & .738 & .508 \\
\multirow{15}{*}{8}   &                           &  3 & .951 & .475 & .213 \\
					  &                           & 5 & .967 & .836 & .148 \\
					  &                           & 7 & .967 & .77 & .262 \\
					  &                           & 9 & .984 & .754 & .262 \\
					  &                           & 11 & .967 & .787 & .115 \\
					  &                           & 30 & .967 & .82 & .377 \\
					  &                           & 50 & .984 & .803 & .295 \\
					  &                           & 70 & .967 & .852 & .328 \\
					  &                           & 90 & .967 & .852 & .377 \\
					  &                           & 110 & .984 & .852 & .311 \\
					  &                           & 300 & .984 & .836 & .344 \\
					  &                           & 500 & .984 & .836 & .344 \\
					  &                           & 700 & .984 & .803 & .361 \\
					  &                           & 900 & .984 & .82 & .361 \\
					  &                           & 1100 & .984 & .836 & .361 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

The table \ref{table:breast_cancer_random_forest} shows the results obtained by a Random Forest on the Breast dataset. The field \texttt{\#Tree} is divided into \texttt{Set} an \texttt{Best CV}. The filed \texttt{Set} indicates that the number of trees in the RF has been specified manually. \texttt{Best CV} instead indicates that the number of estimators has been chosen based on the maximum accuracy obtained with a cross-validation performed with $k$-Fold with $k = 5$ on the train set.


==> 05-conclusion.tex <==
%!TEX root=./paper.tex

\section{Conclusion}
\label{sec:conclusion}
